Estimation with missing not at random binary outcomes via exponential tilts

We study the problem of missing not at random (MNAR) datasets with binary outcomes. We propose an exponential tilt based approach that bypasses any knowledge on 'nonresponse instruments' or 'shadow variables' that are usually required for statistical estimation. We establish a sufficient condition for identifiability of tilt parameters and propose an algorithm to estimate them. Based on these tilt parameter estimates, we propose importance weighted and doubly robust estimators for any mean functions of interest, and validate their performances in a synthetic dataset. In an experiment with the Waterbirds dataset, we utilize our tilt framework to perform unsupervised transfer learning, when the responses are missing from a target domain of interest, and achieve a prediction performance that is comparable to a gold standard.

==> YK-macros.tex <==

\def\Avar{{\sf Avar}}
\def\abs#1{\left|#1\right|}
\def\aff{{\sf aff}}
\def\argmin{{\arg\min}}
\def\argmax{{\arg\max}}
\def\avar{{\sf avar}}

\def\bA{\mathbf{A}}
\def\bB{\mathbf{B}}
\def\bC{\mathbf{C}}
\def\bD{\mathbf{D}}
\def\bE{\mathbf{E}}
\def\bF{\mathbf{F}}
\def\bff{\mathbf{f}}
\def\bG{\mathbf{G}}
\def\bH{\mathbf{H}}
\def\bI{\mathbf{I}}
\def\bJ{\mathbf{J}}
\def\bK{\mathbf{K}}
\def\bL{\mathbf{L}}
\def\bM{\mathbf{M}}
\def\bN{\mathbf{N}}
\def\bO{\mathbf{O}}
\def\bP{\mathbf{P}}
\def\bQ{\mathbf{Q}}
\def\bR{\mathbf{R}}
\def\bS{\mathbf{S}}
\def\bT{\mathbf{T}}
\def\bU{\mathbf{U}}
\def\bV{\mathbf{V}}
\def\bW{\mathbf{W}}
\def\bX{\mathbf{X}}
\def\bY{\mathbf{Y}}
\def\bZ{\mathbf{Z}}

\def\bGamma{{\boldsymbol\Gamma}}
\def\bDelta{{\boldsymbol\Delta}}
\def\bTheta{{\boldsymbol\Theta}}
\def\bLambda{{\boldsymbol\Lambda}}
\def\bXi{{\boldsymbol\Xi}}
\def\bPi{{\boldsymbol\Pi}}
\def\bSigma{{\boldsymbol\Sigma}}
\def\bUps{{\boldsymbol\Upsilon}}
\def\bPhi{{\boldsymbol\Phi}}
\def\bPsi{{\boldsymbol\Psi}}
\def\bOmega{{\boldsymbol\Omega}}

\def\ba{\mathbf{a}}
\def\bb{\mathbf{b}}
\def\bc{\mathbf{c}}
\def\bbd{\mathbf{d}}
\def\bd{{\sf bd}}
\def\be{\mathbf{e}}
\def\bbf{\mathbf{f}}
\def\bg{\mathbf{g}}
\def\bh{\mathbf{h}}
\def\bi{\mathbf{i}}
\def\bj{\mathbf{j}}
\def\bk{\mathbf{k}}
\def\bl{\mathbf{l}}
% \def\bm{\mathbf{m}}
\def\bn{\mathbf{n}}
\def\bo{\mathbf{o}}
\def\bp{\mathbf{p}}
\def\bq{\mathbf{q}}
\def\br{\mathbf{r}}
\def\bs{\mathbf{s}}
\def\bt{\mathbf{t}}
\def\bu{\mathbf{u}}
\def\bv{\mathbf{v}}
\def\bw{\mathbf{w}}
\def\bx{\mathbf{x}}
\def\by{\mathbf{y}}
\def\bz{\mathbf{z}}

\def\balpha{{\boldsymbol\alpha}}
\def\bbeta{{\boldsymbol\beta}}
\def\bgamma{{\boldsymbol\gamma}}
\def\bdelta{{\boldsymbol\delta}}
\def\beps{{\boldsymbol\epsilon}}
\def\bveps{{\boldsymbol\varepsilon}}
\def\bzeta{{\boldsymbol\zeta}}
\def\bfeta{{\boldsymbol\eta}}
\def\btheta{{\boldsymbol\theta}}
\def\bvtheta{{\boldsymbol\vartheta}}
\def\biota{{\boldsymbol\iota}}
\def\bkappa{{\boldsymbol\kappa}}
\def\blambda{{\boldsymbol\lambda}}
\def\bmu{{\boldsymbol\mu}}
\def\bnu{{\boldsymbol\nu}}
\def\bxi{{\boldsymbol\xi}}
\def\bpi{{\boldsymbol\pi}}
\def\brho{{\boldsymbol\rho}}
\def\bvrho{{\boldsymbol\varrho}}
\def\bsigma{{\boldsymbol\sigma}}
\def\btau{{\boldsymbol\tau}}
\def\bups{{\boldsymbol\upsilon}}
\def\bphi{{\boldsymbol\phi}}
\def\bvphi{{\boldsymbol\varphi}}
\def\bpsi{{\boldsymbol\psi}}
\def\bomega{{\boldsymbol\omega}}

\def\bbA{\mathbb{A}}
\def\bbB{\mathbb{B}}
\def\bbC{\mathbb{C}}
\def\bbD{\mathbb{D}}
\def\bbE{\mathbb{E}}
\def\bbF{\mathbb{F}}
\def\bbG{\mathbb{G}}
\def\bbH{\mathbb{H}}
\def\bbI{\mathbb{I}}
\def\bbJ{\mathbb{J}}
\def\bbK{\mathbb{K}}
\def\bbL{\mathbb{L}}
\def\bbM{\mathbb{M}}
\def\bbN{\mathbb{N}}
\def\bbO{\mathbb{O}}
\def\bbP{\mathbb{P}}
\def\bbQ{\mathbb{Q}}
\def\bbR{\mathbb{R}}
\def\bbS{\mathbb{S}}
\def\bbT{\mathbb{T}}
\def\bbU{\mathbb{U}}
\def\bbV{\mathbb{V}}
\def\bbW{\mathbb{W}}
\def\bbX{\mathbb{X}}
\def\bbY{\mathbb{Y}}
\def\bbZ{\mathbb{Z}}


\def\ccA{\mathscr{A}}
\def\ccB{\mathscr{B}}
\def\ccC{\mathscr{C}}
\def\ccD{\mathscr{D}}
\def\ccE{\mathscr{E}}
\def\ccF{\mathscr{F}}
\def\ccG{\mathscr{G}}
\def\ccH{\mathscr{H}}
\def\ccI{\mathscr{I}}
\def\ccJ{\mathscr{J}}
\def\ccK{\mathscr{K}}
\def\ccL{\mathscr{L}}
\def\ccM{\mathscr{M}}
\def\ccN{\mathscr{N}}
\def\ccO{\mathscr{O}}
\def\ccP{\mathscr{P}}
\def\ccQ{\mathscr{Q}}
\def\ccR{\mathscr{R}}
\def\ccS{\mathscr{S}}
\def\ccT{\mathscr{T}}
\def\ccU{\mathscr{U}}
\def\ccV{\mathscr{V}}
\def\ccW{\mathscr{W}}
\def\ccX{\mathscr{X}}
\def\ccY{\mathscr{Y}}
\def\ccZ{\mathscr{Z}}

\def\Ber{{\sf Ber}}
\def\bin{{\sf bin}}

\def\cA{\mathcal{A}}
\def\cB{\mathcal{B}}
\def\cC{\mathcal{C}}
\def\cD{\mathcal{D}}
\def\cE{\mathcal{E}}
\def\cF{\mathcal{F}}
\def\cG{\mathcal{G}}
\def\cH{\mathcal{H}}
\def\cI{\mathcal{I}}
\def\cJ{\mathcal{J}}
\def\cK{\mathcal{K}}
\def\cL{\mathcal{L}}
\def\cM{\mathcal{M}}
\def\cN{\mathcal{N}}
\def\cO{\mathcal{O}}
\def\cP{\mathcal{P}}
\def\cQ{\mathcal{Q}}
\def\cR{\mathcal{R}}
\def\cS{\mathcal{S}}
\def\cT{\mathcal{T}}
\def\cU{\mathcal{U}}
\def\cV{\mathcal{V}}
\def\cW{\mathcal{W}}
\def\cX{\mathcal{X}}
\def\cY{\mathcal{Y}}
\def\cZ{\mathcal{Z}}

\def\cat{{\sf cat}}
\def\Cov{{\sf Cov}}
\def\cov{{\sf cov}}
\def\card{{\bf card}}
\def\cf{{\it cf.}}
\def\cl{{\sf cl}}
\def\complex{{\bbC}}
\def\cone{{\sf cone}}
\def\conv{{\sf conv}}
\def\deq{\overset{d}{=}}
\def\det{{\sf det}}
\def\diag{{\sf diag}}
\def\diam{{\sf diam}}
\def\dist{{\sf dist}}
\def\dom{{\sf dom}}
\def\doop{{\sf do}}
\def\dto{\overset{\sf d}{\to}}
\def\Ex{{\bbE}}
\def\Exp{{\sf Exp}}
\def\exp{{\sf exp}}
\def\eg{{\it e.g.}}
\def\epi{{\sf epi}}
\def\eps{{\epsilon}}
\def\etc{{\it etc.}}
\def\ie{{\it i.e.}}
\def\iid{{\sf iid}}
\def\ind{{\sf ind}}
\def\intr{{\sf int}}
\def\integers{{\bbZ}}

\def\halpha{\widehat{\balpha}}
\def\hbeta{\widehat{\bbeta}}
\def\hdelta{\widehat{\bdelta}}
\def\hGamma{\widehat{\bGamma}}
\def\hgamma{\widehat{\bgamma}}
\def\hmu{\widehat{\bmu}}
\def\hSigma{\widehat{\bSigma}}
\def\hsigma{\widehat{\bsigma}}
\def\hTheta{\widehat{\bTheta}}
\def\htheta{\widehat{\btheta}}
\def\hw{\widehat{\bw}}

\def\KL{{\sf KL}}
\def\ker{{\sf ker}}
\def\lspan{{\sf span}}
\def\maximize{{\sf maximize}}
\def\med{{\sf med}}
\def\minimize{{\sf minimize}}
\def\norm#1{\left\|#1\right\|}
\def\ones{\mathbf{1}}
\def\Poi{{\sf Poi}}
\def\Pr{{\bbP}}
\def\peq{\overset{\sf p}{=}}
\def\plim{{\sf plim}}
\def\proj{{\sf proj}}
\def\prox{{\sf prox}}
\def\pto{\overset{\sf p}{\to}}
\def\ran{{\sf ran}}
\def\rank{{\sf rank}}
\def\reals{{\bbR}}
\def\relint{{\sf relint}}
\def\sign{{\sf sign}}
\def\supp{{\sf supp}}
\def\symm{{\bbS}}

\def\st{\textrm{subject to}}
\def\tr{{\sf tr}}
\def\tube{{\sf tube}}
\def\TV{{\sf TV}}
\def\unif{{\sf unif}}
\def\Var{{\sf Var}}
\def\var{{\sf var}}
\def\vct{{\sf vec}}
\def\veps{\varepsilon}
\def\vol{{\sf vol}}
\def\zeros{\mathbf{0}}


==> YK-thm-macros.tex <==

\newtheorem{theorem}{Theorem}[section]
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{condition}[theorem]{Condition}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{model}[theorem]{Model}
% \newenvironment{proof}{\noindent {\sc Proof:}}{$\Box$ \medskip} 
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{remark}[theorem]{Remark}


\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage{lineno}
\newcommand{\COMMENTV}[2][.4\linewidth]{%
  \leavevmode\hfill\makebox[#1][l]{~~ //~#2}}

 

==> sections/asymp.tex <==
\subsection{Asymptotic distributions}
\label{sec:asym-distr}

In this section, we discuss asymptotic distributions for IW and DR estimators. Both the estimators are sample averages with respect to appropriate scores, as
\begin{equation}\label{eq:score-rep}
    \begin{aligned}
        & \textstyle \widehat \mu_{0, \psi} = \frac{1}{n} \sum_{i = 1}^n\delta_{0, \psi}(X_i, Y_i, R_i; \widehat \theta, \widehat \xi), ~~~ \widehat \mu_{\psi} = \frac{1}{n} \sum_{i = 1}^n\delta_{\psi}(X_i, Y_i, R_i; \widehat \theta, \widehat \xi), ~~ \psi \in \{ \text{IW}, \text{DR}\} \\
&  \text{where,} \textstyle ~~    \delta_{0, \text{IW}}(X_i, Y_i, R_i; \widehat \theta, \widehat \xi) = \frac{R_i}{\widehat \pi_r} \omega(X_i, Y_i; \widehat \theta, \widehat \xi) \tau(X_i, Y_i)   , \\
& \textstyle \delta_{ \text{IW}}(X_i, Y_i, R_i; \widehat \theta, \widehat \xi) = {R_i \big \{ 1 + \frac{1- \widehat \pi_r}{\widehat \pi_r}  \omega(X_i, Y_i; \widehat \theta) \big \} \tau(X_i, Y_i)} \\
& \textstyle\delta_{0, \text{DR}}(X_i, Y_i, R_i; \widehat \theta, \widehat \xi) = \frac{R_i}{\widehat \pi_r} \omega(X_i, Y_i; \widehat \theta) \{\tau(X_i, Y_i) -  m_{0, \tau} (X_i; \widehat \theta, \widehat \xi)\} +  \frac{1 - R_i}{1 - \widehat \pi_r}  m_{0, \tau}(X_i; \widehat \theta, \widehat \xi)\\
& \textstyle\delta_{\text{DR}}(X_i, Y_i, R_i; \widehat \theta, \widehat \xi) = R_i \{\frac{1 - \widehat \pi_r}{\widehat \pi_r} + \widehat \omega(X_i, Y_i)\}  \{ \tau(X_i, Y_i) -  m_{0, \tau}(X_i; \widehat \theta, \widehat \xi)\} +    m_{0, \tau}(X_i; \widehat \theta, \widehat \xi)
    \end{aligned}
\end{equation} 
If the $\{(X_i, Y_i, R_i)\}_{i = 1}^n$ is the sample that is not used for calculating $\widehat \theta$ and $\widehat \xi$ , \ie these parameters are estimated on a separate data split, then a simple application of the central limit theorem and Slutsky's lemma yields the following asymptotic distributions: 
\begin{equation}
    \begin{aligned}
        & \sqrt{n} \big(\widehat \mu_{0, \psi} - \Ex[\delta_{0, \psi}(X_i, Y_i, R_i;  \theta^\star,  \xi^\star)]\big)    \stackrel{\text{d}}{\longrightarrow} \cN \big(0, \var[\delta_{0, \psi}(X_i, Y_i, R_i;  \theta^\star,  \xi^\star)] \big)\,,\\
        & \sqrt{n} \big(\widehat \mu_{\psi} - \Ex[\delta_{ \psi}(X_i, Y_i, R_i;  \theta^\star,  \xi^\star)]\big)    \stackrel{\text{d}}{\longrightarrow} \cN \big(0, \var[\delta_{ \psi}(X_i, Y_i, R_i;  \theta^\star,  \xi^\star)] \big)\,,
    \end{aligned}
\end{equation} as $n \to \infty$ for both $\psi \in \{ \text{IW}, \text{DR}\}$, where $\stackrel{\text{d}}{\longrightarrow}$ denotes convergence in distribution. Now, if $\Ex[\delta_{0, \psi}(X_i, Y_i, R_i;  \theta^\star,  \xi^\star)] = \mu_0$ and $\Ex[\delta_{ \psi}(X_i, Y_i, R_i;  \theta^\star,  \xi^\star)] = \mu$, \ie\  if the asymptotic biases are zero (see Theorem \ref{thm:double-robustness} for more discussion on asymptotic bias), then these asymptotic distributions can be utilized for constructing confidence intervals for $\mu_0$ and $\mu$. 



